JUMPER: Learning When to Make Classification Decisions in Reading

In early years, text classification is typically accomplished by feature-based machine learning models; recently, deep neural networks, as a powerful learning machine, make it possible to work with raw input as the text stands. However, exiting end-to-end neural networks lack explicit interpretation of the prediction. In this paper, we propose a novel framework, JUMPER, inspired by the cognitive process of text reading, that models text classification as a sequential decision process. Basically, JUMPER is a neural system that scans a piece of text sequentially and makes classification decisions at the time it wishes. Both the classification result and when to make the classification are part of the decision process, which is controlled by a policy network and trained with reinforcement learning. Experimental results show that a properly trained JUMPER has the following properties: (1) It can make decisions whenever the evidence is enough, therefore reducing total text reading by 30-40% and often finding the key rationale of prediction. (2) It achieves classification accuracy better than or comparable to state-of-the-art models in several benchmark and industrial datasets.

==> Learning.tex <==
\section{Learning}
Actually, in the scenarios of text classification, there are few annotations to show where the pattern is, so the immediate supervision is not available. Thus we could use policy gradient method to address it. \jumperb samples an action from distribution(in fomulation $(9)$) given by PolicyNet, and only one jump in each slot is allow according the constrain in Symbolic Layer. The parameters of \jumperb (denoted $\Theta$) include all the parameters in  Sentence Encoder and Controller. They are trained with reinforcement learning, and the supervision is given as rewards during the decision process, for which an extreme case is to give the final reward at the end of the decision process by comparing the prediction with the ground truth, e.g.,  \vspace{-4pt}
\begin{equation}
R_{final}^{(i)}=\textsf{equal}(\textsf{y}_{i},\mathcal{Y}_{i})  
\end{equation} 
where the $\textsf{equal}(\textsf{y}_{i},\mathcal{Y}_{i})$ measures the equivalence between the prediction  $\textsf{y}_{i}$ and the ground truth $\mathcal{Y}_{i}$ and $i$ is the index of data. However, there are some difficulties to sample a valuable solution when the length of sentence is long and the key pattern is at the very bottom. Here an immediate reward is given to the agent to encourage it to not jump until the key pattern appears.
\begin{equation}
R_{nojump}^{(i,t)}=\left\{
\begin{aligned}
r,  \;\;\;&\text{if $ s_t = 0$ } \\
0,   \;\;\;&\text{else  }\\ 
\end{aligned}
\right.
\label{e:reward_zero} \vspace{-4pt}
\end{equation} 
where $R_{nojump}^{(i,t)}$ is the immediate reward of data $i$ at t step. Thus the accumulated reward at step $t$ can be fomulated as:
\begin{equation}
R_{t:T_{jump}^{(i)}}^{(i)} = \sum_{t'=t}^{T_{jump}^{(i)}} \gamma^{t'-t}R_{nojump}^{(i,t')} + R_{final}^{(i)}  
\end{equation} 
where $\gamma$ is the discounting rate, $ T_{jump}^{(i)}$ denotes the step of jumping.  We can use any policy search algorithm to maximize the expected total reward. With the commonly used REINFORCE~\cite{williams92-reinforce} for training, the gradient is given by  \vspace{-4pt}
\begin{align}
\nabla_\Theta\mathcal{J}(\Theta) &= \mathbb{E}_{\pi_\theta}\left[\nabla_\Theta \log \pi_\Theta \left( a_t^{i} | s_t^i \right) R_{t:T}^{(i)} \right] \\  &\approx -\frac{1}{NT_i}\sum_i^N\sum_{t=1}^{T_{jump}^{(i)}} \nabla_\Theta \log \pi_\Theta \left( a_t^{i} | s_t^i \right) R_{t:T_{jump}^{(i)}}^{(i)}. \vspace{-4pt}
\end{align}


==> e1.tex <==
\subsection{Dataset}  \label{s:dataset}
We collect a new 15-task dataset about occupation injury and use two publicly available datasets from \cite{Zhang15-cnnText}  to evaluate our models. They are standard text classification datasets that include news classification, sentiment analysis. Table \ref{tab:data-stat} shows descriptive statistics of datasets. For each dataset, we randomly select 5\% samples from the original training set as the development set.

\begin{table}[h!]
	\center
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\textbf{Data} & $c$ & $N$ & $|V|$ & $|V_{pre}|$ & \emph{Test} \\ \hline
		MR & $2$  & $10662$ &  $18765$ & $16448$ & CV \\ 
		AG &  $4$ &  $11855$ &  $17836$ & $16262$ & $2210$ \\ 
		OI dataset &  $12$  &  $3995$ & $2089$  & None & $500$  \\
		\hline
	\end{tabular}
	\caption{Summary statistics for the datasets after tokenization. $c$: Number of target classes. $N$: Dataset size. $|V|$: Vocabulary size. $|V_{pre}|$: Number of words present in the set of pre-trained word vectors. \emph{Test}: Test set size (CV means there was no standard train/test split and thus 10-fold CV was used).}
	\label{tab:data-stat}
\end{table}

\subsubsection{Occupational Injury Dataset}
We built a dataset including 3995 cases related to industrial injury in Chinese and established an ontology of industrial injury law which is consisted of 59 relevant problems. In other words, each text is annotated with answers for 59 problems respectively. On the right of the Figure \ref{fig:task-example}, it's the translation of the text and the bottom shows three subtasks and corresponding annotations, where the bold text indicates the abbreviation of the subtasks.
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.65\linewidth]{image/ojtask.png}
		\caption{An example of Occupational Injury and three of the subtasks.}\label{fig:task-example}
	\end{figure}
	
In addition, 15 distributed balanced problems are selected to build a dataset for multitask classification, which are divided into training/development/testing set with 2995/500/500 samples. Table \ref{tab:dataset2} summarizes the  class number and majority guess for each problem of the 15 subtasks. The 15 subtasks are relevant to each other, and the composition of their answers can be built as a knowledge graph, which is very important for understanding and knowledge representation.
\begin{table}[h!]
	\centering
	\resizebox{0.5\linewidth}{!}{
		\begin{tabular}{|l|c|c|c|c|}
			\hline
			Subtask & Num of Class & Majority Guess (\%)  \\
			\hline
			\hline
			IsOccuInj &  2 & 85.68 \\
			\hline
			AssoPay  & 2 & 81.75 \\
			\hline
			LaborContr & 2  &  93.22 \\
			\hline
			EndLabor & 3  &  93.67 \\
			\hline
			OnOff & 2  &  93.69 \\
			\hline
			DiseRel & 3  &  99.05 \\
			\hline
			OutForPub & 2  &  99.07 \\
			\hline
			WorkTime & 3  &  79.75 \\
			\hline
			WorkPlace & 3  &  80.60 \\
			\hline
			JobRel & 3  &  91.34 \\
			\hline
			InjIden & 3  &  55.02 \\
			\hline
			ConfirmLevel & 3  &  72.99 \\
			\hline
			Insurance & 3  &  89.66 \\
			\hline
			HaveMedicalFee & 3  &  83.63 \\
			\hline
			Level & 12  &  82.65 \\
			\hline
		\end{tabular} }%\vspace{-2mm}
		\caption{Statistics of Occupational Injury Case dataset. Selected 15 distributed balanced problems.}
		\label{tab:dataset2}
	\end{table}

\subsection{Competitor Methods and Hyperparameters}
There are many models that achieved great performance in text classification and we only choose several typical models to implement them as strong competitors.
\begin{itemize}
	\item \textbf{Non-Restricted \reader}(Non-\reader): We use \readerb without  the Symbolic Layer as a baseline model. While it is little change with former model, the informantion flow may change a lot due to the difference in length of back propagation.
	\item \textbf{Bi-GRU}: classify the text with the features by combining of the two hidden states, which are the final states of a forward GRU and a backward GRU that read the sentences in two opposite directions.
	\item \textbf{CNN}: This model is proposed by \cite{Kim14sent}, with several different kernel sizes of convolution operators to learn sentence representation.
	\item \textbf{Bi-GRU-Maxpool}: \textbf{Bi-GRU} reads the text word by word to extract features, and max pooling layer selects the maximum value over each dimension of the hidden units to form a fixed-size vector for classification(\cite).
\end{itemize}
For all the models we trained, we use Adadelta algorithm
with a learning rate of 0.1 and a exploration rate of 0.2. We use minibatches of size 50 and training is stopped when the learning rate goes under the threshold of $10^{−5}$. For the classifier, we use a multi-layer perceptron with 1 hidden-layer of 20 hidden units. We use opensource GloVe vectors trained on Common Crawl 840B2 with 300 dimensions as fixed word embeddings.

\subsection{Results and discussion}
In this section, we are going to explain results of the experiment and some senseful behaviors in decision process to study the characters of \reader.
\subsubsection{Performance of \jump}
We have annotated the jumping sentence in 1000 texts in the test data of AG News Corpus which is available at deepcurious.ai/data. And we consider the following two metrics in comparing the performance of \readerb and Non-\readerb: 
\vspace{-5pt}
\begin{table*}[h!]
	\centering
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{ll}
			%\hline
			Classification  Accuracy(\textbf{C.A})  & the accuracy of predicting the category. \\ %\hline
			Jumping Accuracy(\textbf{J.A}) & the correct rate of both classification and jumping \\ %\hline
			%Impulsively Jumping Accuracy(\textbf{I.J.A}) & the accuracy of jumping or jumping before location conditioned on predicting correctly \\ %\hline
		\end{tabular}
	}\vspace{-2mm}
	%\caption{Explanation.}\label{tab:Explanation}
	\vspace{-2mm}
\end{table*}

In addition, the answer of which when the infomation is enough for classification varies between people in some entangled case, So we relax some restriction of the second metric: As long as the jumping position is the same as the groundtruth or earlier one step than the groundtruth, it is regarded as correct.

Due to the sequential characteristics of Non-\readerb, it can be also regarded as a decision process when reading sentence by sentence. To be comparable, the jumping location of Non-\readerb is the first time of Non-\readerb changing the prediction. Table \ref{tab:jump-perf} summarizes the results with the two forementioned metrics. Our results show that the \readerb outperforms Non-\readerb by a significant margin in both two metrics. This high reliability of jumping is attributed to the constrain of symbolic layer. It seems that the contrller has learnt to not jump until the infomation is abundant enough.
\begin{table}[h!]
	\center
	\begin{tabular}{|c|c|c|}
		\hline
		\textbf{Model} & \textbf{C.A} & \textbf{J.A} \\ \hline
		\reader & 91.80 & 82.31 \\ 
		Non-\reader & 87.6 & 76.43  \\ 
		\hline
	\end{tabular}
	\caption{Comparation between \readerb and Non-\reader}
	\label{tab:jump-perf}
\end{table}


\subsubsection{Performance of Classification}
We empirically examined \readerb and compared them with some competitors of great value. Table \ref{tab:perf-res} shows the classification accuracies on the four datasets. The row with starred model name indicates the results is quoted, and all else is reproduced by ourselves. The results show that despite the lack of task-specific tuning our model performs surprisingly well, yielding competitive results with previously reported models. \readerb and Non-\readerb use CNN(\cite{Kim14sent}) as the sentence encoder, and have longer range denpendence of patterns due to the RNN style, but there is no decrease in performance with comparasion of CNN. 

Furthermore, Table \ref{tab:perf-res} also shows the average length of sentence($L$) in each dataset and sentence that \readerb reads before the \jumpingb point. The average \jumpingb point of \readerb is significantly shorter than the overall length, which endows the \readerb with the capability of escaping long range dependence and performing on-par with state-of-the-art model.
% The performance of Non-\readerb is always inferior to \readerb.
\begin{table}[h!]
	\center
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\textbf{Model} & \textbf{MR} & \textbf{AG} & \textbf{OI-level} & \textbf{OI-InjIden}  \\ 
		\hline
		BoW &  76.40 & 88.90  &  87.22 & 72.68  \\ 
		\hline
		Bi-GRU & 77.80  & 92.44   &  94.99  & 73.18  \\ 
		\hline
		CNN &  80.80 & 92.51 &  96.24  & 74.94   \\ 
		\hline
		CNN\cite{Kim14sent} &  81.00 & - & - & - \\ 
		\hline
		fasttext(\cite{Joulin16Fasttext}) &  - & 92.50 & - & - \\ 
		\hline
		
		%Bi-GRU-Maxpool & 81.06 y & xxx  & 95.80y  & 75.80y\\
		Non-\reader & 80.23 & 92.15 & 95.28 & 74.72  \\ 
		\hline
		\reader & 80.67  & 92.68 & 97.51  & 77.22  \\
		\hline
		\hline
		$L$ & 2.17  & 3.46 & 4.88  & 4.88  \\
		\hline
		Jumping Point & 1.46  & 2.04 & 3.23  & 2.87  \\

		\hline
	\end{tabular}
	\caption{Test accuracy [\%] on several datasets. All model we realized has been run with the same parameters for all the datasets.}
	\label{tab:perf-res}
\end{table}


\subsubsection{Analysis of \jumping}
The results and learning process of \readerb in AG News Corpus is shown in Figure \ref{fig:jumpb}. \readerb learns quickly in first 100 batches (see figure \ref{fig:jumpb} (a)), and then the correct rate of \jumpb continues to rise slowly at a consistent pace with rising of classification accuracy. The variance of correct rate is larger than the accuracy, which indicates \readerb is exploring when to \jumpb during training.  At the same time, on the condition that \readerb predicts correctly, the percentages of the jumping firstly and jumping finally are also have slight changes during training(seee Figure \ref{fig:jumpb} (b)): the percentage of  jumping firstly is decreasing slightly and the trend of  percentage of  jumping finally is the opposite exactly, which indicates \readerb tends to not \jumpb impulsively and wait.
\begin{figure}[htbp]
	\centering                                                  
	\subfigure[Classification and jump accuracy]{                    %第一张子图
		\begin{minipage}{7cm}
			\centering                                                          %子图居中
			\includegraphics[scale=0.5]{image/jump.eps}               %以pic.jpg的0.5倍大小输出
		\end{minipage}}
	\subfigure[ The proportion of jumping firstly and jumping finally]{
		\begin{minipage}{7cm}
			\centering                                         \includegraphics[scale=0.5]{image/oneshot.eps} 
		\end{minipage}}
	\caption{Jumping behavior of \readerb during training} 
	\label{fig:jumpb}                                           
\end{figure}

\subsubsection{Relevant MultiTask}
We implement \readerb to classify text on several relevant tasks simultaneously, which is a common scenario in real world. Taking task of occupational injury \cite{jingxuan} for example, as illustrated in Figure \ref{fig:task-example}, when coming a question, several subtasks need to be determined so that we can give some concrete suggestions for the question based on several predictions in subtasks.  The little change of \readerb for multitask is that decision of each task is fed back into the next step as inputs. The advantages of \readerb in tackling multitask problem are in two folds: Firstly, the working memory can be used for defferent subtask in different time when reading.  Secondly, decision sharing between relevant multitask may help to solve the difficult subtask.

15 distributed balanced problems are selected to evaluate \readerb and its competitors. Table \ref{tab:multitask-exp} shows us the average classification accuracy in the development set and test set of Ocuupational Injury Dataset respectively. We can find that \readerb equiped with decision sharing(\reader-sharing) achieves best performance, which demonstrates decision sharing helps in this problem of relevant multitasks.
\begin{table}
	\center
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		Model & dev & test \\ \hline
		BoW & 90.9 & 89.98  \\
		Bi-GRU & 91.15 & 90.66\\
		CNN & 92.94 & 92.30 \\ 
		Non-\reader & 92.32 &  91.14 \\ 
		\reader & 92.82& 92.51 \\
		\reader-sharing & 93.03 & 92.63 \\
		\hline
	\end{tabular}
	\caption{The mean test accuracy (\%) on OI dataset}
	\label{tab:multitask-exp}
\end{table}

\subsubsection{Case Study}
To get an intuitive understanding of how \readerb makes decision during the process of reading and as an interpretation of relations between jumping and rationanle, we use histogram  to plot the probability of taking action for some texts in both AG and MR datasets. We randomly selected two pieces of news from the AG test set and one review from MR test set for example. As shown in Figure \ref{f:showcase}, in the first case, the confidence in class 'sports' rises along reading and the model jumps when reading at second sentence, without reading the rest sentences. In the third case, which is for sentiment classification, the model firstly puts a fraction of confidence to class 'positive', and when it reads 'however', it give a larger probability to class 'negative', but still hasn't jumpped. When it reads the last sentence, it decides to jump to class 'positive'. We find that the model majorly learns to capture some key sentences in the text that indicate strongly on the topic or sentiment behind the sentence. 
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.9\textwidth]{image/agexample.png}
	\caption{Histogram of decision distribution in AG News Corpus and MR Reviews.}
	\label{f:showcase}
\end{figure}
For most of the texts composed of short sentences, the model manages to locate the key factors and jump, but for the texts composed of long sentences or sentences with no triggers to decompose the meaning groups, \readerb degenerates into a normal classifier. 
